Scattering from time-modulated subwavelength resonators

We consider wave scattering from a system of highly contrasting resonators with time-modulated material parameters. In this setting, the wave equation reduces to a system of coupled Helmholtz equations that models the scattering problem. We consider the one-dimensional setting. In order to understand the energy of the system, we prove a novel higher-order discrete, capacitance matrix approximation of the subwavelength resonant quasifrequencies. Further, we perform numerical experiments to support and illustrate our analytical results and show how periodically time-dependent material parameters affect the scattered wave field.

==> cuts.tex <==

\begin{thm} \label{thm3.1}
    Consider a single-resonator system, \textit{i.e.} $N=1$, where the resonator is of length $\ell$. As $\delta\to0$, the two subwavelength quasifrequencies $\omega$ of (\ref{eq:1DL_system})  are, at leading order, the quasifrequencies of the ordinary differential equation
    \begin{align}\label{eq:cap_1D_N1}
        \frac{2}{v_0}\frac{\mathrm{d}}{\mathrm{d}t}c(t)+\frac{\ell}{\delta(v_{\mathrm{r}})^2}\frac{\mathrm{d}}{\mathrm{d}t}\frac{1}{\kappa(t)}\frac{\mathrm{d}}{\mathrm{d}t}c(t)=0.
    \end{align}
\end{thm}
\begin{proof}
    Let the resonator be given by $D:=(x^-,x^+)$.  From the differential equation and the radiation condition in the far-field, the exterior solution is given by
    \begin{align}\label{eq:vn_N1_simpl}
        v_n^{\mathrm{sc}}(x)=\begin{cases}
            \beta^0_n\mathrm{e}^{-\mathrm{i}k^{(n)}x},&\forall\,x\in(-\infty,x^-],\\
            \alpha^1_n\mathrm{e}^{\mathrm{i}k^{(n)}x},&\forall\,x\in [x^+,\infty),      \end{cases}
    \end{align}
    for constants $\beta^0_n$ and $\alpha^1_n$. Inside $D$, we have $v_n^{\mathrm{sc}}(x)=c_n+
    O(\delta^{(1-\gamma)/2})$ for some constant $c_n$ and $0<\gamma <1$ \cite{erik_JCP}.
    \par
    The continuity condition at the boundaries implies
    \begin{align*}
        \beta_n^0=c_n\mathrm{e}^{\mathrm{i}k^{(n)}x^-},\quad \alpha_n^1=c_n\mathrm{e}^{-\mathrm{i}k^{(n)}x^+}.
    \end{align*}
    % Upon expansion in $x$ to order $\delta$,
    Using (\ref{eq:vn_N1_simpl}), we arrive at
    \begin{align}\label{eq:I_vn_1}
        I_{\partial D}[v_n^{\mathrm{sc}}]=-\mathrm{i}k^{(n)}c_n(\mathrm{e}^{\mathrm{i}k^{(n)}x^-}+\mathrm{e}^{-\mathrm{i}k^{(n)}x^+})=-2 \mathrm{i}k^{(n)}c_n+O(\delta).
    \end{align}\par 
    Next, using the transmission conditions and (\ref{eq:1DL_system}) we obtain
    \begin{equation}\label{eq:I_vn_2}
    \begin{split}
    I_{\partial D} [v_n^{\mathrm{sc}}] &= \frac{1}{\delta} \left(\frac{\mathrm{d} v_{n}^{\mathrm{sc}}}{\mathrm{d} x} \bigg\vert_+(x^-) - \frac{\mathrm{d} v_{n}^{\mathrm{sc}}}{\mathrm{d} x} \bigg\vert_-(x^+) \right)\\
    & = \frac{1}{\delta} \int_{x^-}^{x^+} \frac{\mathrm{d}^2v_{n}^{\mathrm{sc}}}{\mathrm{d} x^2}(x)\, \mathrm{d} x \\
    & =  -\frac{1}{\delta} \int_{x^-}^{x^+}  \frac{\rho_{\mathrm{r}}(\omega+n\Omega)^2}{\kappa_{\mathrm{r}}} v_{1,n}^{**}(x)  \,\mathrm{d} x.
\end{split} 
\end{equation}
Equating (\ref{eq:I_vn_2}) and (\ref{eq:I_vn_1}) yields
\begin{equation}
   \label{eq:I_vn_3} -2\mathrm{i}k^{(n)}c_n=\ell\frac{\omega+n\Omega}{\delta(v_{\mathrm{r}})^2}\sum\limits_{m=-\infty}^{\infty} k_{m}(\omega+(n-m)\Omega)c_{n-m}.
\end{equation}
Defining the function
\begin{equation*}
    c(t):=\sum\limits_{n=-\infty}^{\infty}c_n\mathrm{e}^{-\mathrm{i}(\omega+n\Omega )t}
\end{equation*}
allows us to conclude that $c(t)$ satisfies the differential equation (\ref{eq:cap_1D_N1}). 
\end{proof}
